Matching with multiple criteria and its application to health disparities research

Matching is a popular nonparametric covariate adjustment strategy in empirical health services research. Matching helps construct two groups comparable in many baseline covariates but different in some key aspects under investigation. In health disparities research, it is desirable to understand the contributions of various modifiable factors, like income and insurance type, to the observed disparity in access to health services between different groups. To single out the contributions from the factors of interest, we propose a statistical matching methodology that constructs nested matched comparison groups from, for instance, White men, that resemble the target group, for instance, black men, in some selected covariates while remaining identical to the white men population before matching in the remaining covariates. Using the proposed method, we investigated the disparity gaps between white men and black men in the US in prostate-specific antigen (PSA) screening based on the 2020 Behavioral Risk Factor Surveillance System (BFRSS) database. We found a widening PSA screening rate as the white matched comparison group increasingly resembles the black men group and quantified the contribution of modifiable factors like socioeconomic status. Finally, we provide code that replicates the case study and a tutorial that enables users to design customized matched comparison groups satisfying multiple criteria.

==> sections/3.tripartite_with_old.tex <==
\section{From bipartite to tripartite}

% motivation for tripartite: more generalized refined balance
% definition of randomization balances over all covariates

\subsection{Basic network structure}\label{subsec: tripartite structure}
More recently, \citet{zhang2021matching} proposed a minimum-cost network flow algorithm built upon a tripartite graph for multivariate matching. The network infrastructure of a generic tripartite network is depicted in Figure \ref{fig: tripartite network} and can be formalizes as follows. A directed graph $\mathcal{G}$ is a set of vertices $\mathcal{V}$ and a set of directed edges $\mathcal{E}$ consisting of ordered pairs $e = (v_1, v_2)$ of distinct vertices. A total of $A$ units, $\mathcal{A} = \{\tau_1, \dots, \tau_A\}$, are represented in the far left part of the network by nodes labeled $\tau_a$, $a = 1, \dots, A$. In parallel, a total of $B$ units, $\mathcal{B} = \{\omega_1, \dots, \omega_B\}$, are represented in the far right part of the network by nodes labeled $\omega_b$, $b = 1, \dots, B$. Finally, a total of $C$ units, $\mathcal{C} = \{\gamma_1, \dots, \gamma_C\}$, occur twice in the network and are represented by nodes labeled $\gamma_c$ and their mirror copies $\overline\gamma_c$, $c = 1, \dots, C$. When adopting this tripartite network structure in a statistical matching problem, as opposed to a standard bipartite network structure depicted in Figure \ref{fig: bipartite plot}, the goal is to select a subset of units $\mathcal{C}'$ from $\mathcal{C}$ so that $\mathcal{C}'$ resemble units in both $\mathcal{A}$ and $\mathcal{B}$, but possibly in different ways. Write $|S|$ for the number of elements of a finite set $S$, so $|\mathcal{A}|=A$, $|\mathcal{B}|=B$ and $|\mathcal{C}|=C$. We require that $C > \max\{A, B\}$ and that $C > \text{LCM}(A, B)$, where LCM denotes the least common multiple of A and B.

%and $B$ units $\mathcal{B} = \{\gamma_1, \dots, \gamma_B\}$ are represented by nodes labeled $\gamma_b$, $b = 1, \dots, B$. In parallel, a copy of $\gamma_b$ denoted as $\overline\gamma_c$. Finally, $Z$ units $\mathcal{Z} = \{\omega_1, \dots, \omega_Z\}$ are represented in the far right network, by nodes labeled $\omega_z$, $z = 1, \dots, Z$. Suppose we are constructing a 1-to-1-to-1 matched set where each of the $Z \leq T$ units both on the far left and right is to be matched to one of the $C \geq T$ units in the middle. And Figure \ref{fig: tripartite network} provides a basic illustration of this network.

There is a source vertex $\xi$ and a sink vertex $\overline{\xi}$, so that the network consists of $|\mathcal{V}| = A + 2C + B + 2$ total vertices:
\begin{equation*}
    \mathcal{V} = \left\{\xi, \tau_1, \dots, \tau_A, \gamma_1, \dots, \gamma_C, \overline\gamma_1, \dots, \overline\gamma_C, \omega_1, \dots, \omega_B,  \overline\xi\right\}.
\end{equation*}
This tripartite network consists of the following edges:
\begin{equation*}
    \mathcal{E} = \left\{(\xi, \tau_a), (\tau_a, \gamma_c), (\gamma_c, \overline\gamma_c), (\overline\gamma_c, \omega_b), (\omega_b, \overline\xi), ~a = 1, \dots, A,~c = 1, \dots, C, ~b = 1, \dots, B \right\}.
\end{equation*}
Thus, there are a total of $|\mathcal{E}| = A + C + B + AC + CB$ edges.

%Similarly as mentioned in Section \ref{sec: matching in bipartite graph}, we transform a statistical matching problem into a minimum-cost network flow problem by structuring metaphorical terminology of the capacity and cost on each edge.
Let $\text{cap}(e)\geq 0$ denote the capacity of an edge $e \in \mathcal{E}$. In the basic network structure depicted in Figure \ref{fig: tripartite network}, all edges of the form $e(\xi, \tau_a)$, $a = 1, \dots, A$, have capacity $\kappa = \text{LCM(A, B)}/A$. Analogously, all edges of the form $e(\overline\gamma_c, \overline{\xi})$, $c = 1, \dots, C$, have capacity $\kappa' = \text{LCM(A, B)}/B$. All other edges, including those of the form $e(\tau_a, \gamma_c)$, $e(\gamma_c, \overline\gamma_c)$, and $e(\overline\gamma_c, \omega_b)$, $a = 1 \dots, A$, $b = 1, \dots, B$, and $c = 1, \dots, C$, all have capacity $1$. 

A feasible flow $f(\cdot)$ is a function that assigns a nonnegative integer to each edge $e \in \mathcal{E}$, such that
\begin{itemize}
    \item[(i)] $0 \leq f(e) \leq \text{cap}(e),~ \text{for } e\in\mathcal{E}$,
    \item[(ii)] all flow units supplied at $\xi$ are absorbed at $\overline\xi$, i.e., $\sum_{a = 1}^A f\{(\xi, \tau_a)\} = \sum_{b = 1}^B f\{(\omega_b, \overline\xi)\} = \text{LCM}(A, B)$,
    \item[(iii)] the flow into each vertex equals the flow out from each vertex, i.e., write $\mathcal{E}^\prime \subset \mathcal{E}$ for the set of edges that include neither the source $\xi$ nor the sink $\overline\xi$, then $\sum_{(a,b)\in\mathcal{E}^\prime} f\{(a,b)\} = \sum_{(b,c)\in\mathcal{E}^\prime} f\{(b,c)\}$ for all $b \in \mathcal{V}\backslash\{\xi, \overline\xi\}$.
\end{itemize}

A feasible flow produces a feasible match. Because all edges of the form $e(\tau_a, \gamma_c)$ and $e(\overline\gamma_c, \omega_b)$ have capacity $1$, quantities of the form $f(\tau_a, \gamma_c)$ and $f(\overline\gamma_c, \omega_b)$ all take an integer value of either $0$ or $1$. Formally, the matched sample $\mathcal{M}(f)$ is defined by
\begin{equation*}
    \mathcal{M}(f) = \left\{(\tau_a, \gamma_c), (\overline\gamma_c, \omega_b)\in \mathcal{E}: f\{(\tau_a, \gamma_c)\} = f(\overline\gamma_c, \omega_b)= 1\right\}.
\end{equation*}
Lastly, $\mathfrak{M} = \left\{ \mathcal{M}(f): \text{for some feasible } f \right\}$ denotes the set of all feasible matched samples. According to the tripartite network and edges' associated capacities in the network, we are constructing one matched sample via conducting two optimal bipartite matching at one shot: a $1$-to-$\kappa$-match facilitated by the left part of the network and a $1$-to-$\kappa'$-match facilitated by the right part of the network.

\subsection{Cost and optimal matched sample}
\label{subsec: cost}
The cost of each edge helps select the matched sample satisfying the desired features of the problem. Let $\text{cost}(e)$ denote the cost associated with edge $e \in \mathcal{E}$. In the basic network structure depicted in Figure \ref{fig: tripartite network}, we let $\text{cost}\{(\xi, \tau_a)\} = \text{cost}\{(\gamma_c, \overline\gamma_c)\} = \text{cost}\{ \omega_b, \overline\xi\} = 0$ for $a = 1, \dots, A$, $b = 1, \dots, B$ and $c = 1, \dots, C$. Each edge of the form $e(\tau_a, \gamma_c)$ is associated with a cost $\delta_{\tau_a, \gamma_c} \geq 0$. We equate $\delta_{\tau_a, \gamma_c}$ to a measure of similarity between unit $\tau_a$ and unit $\gamma_c$, that is,
\begin{align*}
    \text{cost}\{(\tau_a, \gamma_c)\} &= \delta_{\tau_a, \gamma_c}, ~\forall~e(\tau_a, \gamma_c) \in \mathcal{E}.
\end{align*}
Analogously, each edge of the form $e(\overline\gamma_c, \omega_b)$ is associated with a cost $\Delta_{\overline\gamma_c, \omega_b} \geq 0$ which is equal to a measure of the similarity between unit $\omega_b$ and unit $\gamma_c$, that is,
\begin{align*}
    \text{cost}\{(\overline\gamma_c, \omega_z)\} &= \Delta_{\overline\gamma_c, \omega_b}, ~\forall~e(\overline\gamma_c, \omega_b) \in \mathcal{E}.
\end{align*}
Lastly, we let a parameter $\lambda \geq 0$ control the relative importance of the two costs, so that the cost of a feasible flow $f$ in the network becomes:
\begin{equation}\label{eq: tripartite flow cost}
    \text{cost}(f) = \sum_{(\tau_a, \gamma_c) \in \mathcal{M}(f)}\delta_{\tau_a, \gamma_c} + 
    \lambda \Big\{ \sum_{(\overline\gamma_c, \omega_b) \in \mathcal{M}(f)}\Delta_{\overline\gamma_c, \omega_b} \Big\}.
\end{equation}
A minimum cost flow is a feasible flow $g(\cdot)$ such that $\text{cost}(g) \leq \text{cost}(f)$ for every feasible flow $f(\cdot)$.  

%and in other words, it selects $kT$ distinct controls that minimize the weighted sum of two types of cost in the network.

%such that
%\begin{align*}
%    \text{cost}\{(\tau_t, \gamma_c)\} &= \delta_{\tau_t, \gamma_c}, ~\text{for } (\tau_t, \gamma_c) \in \mathcal{E}\\
%    \text{cost}\{(\overline\gamma_c, \omega_z)\} &= \lambda  \Delta_{\overline\gamma_c, \omega_z}, ~\text{for } (\overline\gamma_c, \omega_z) \in \mathcal{E}\\
%    \text{cost}(e) &= 0, ~\text{for all other } e \in \mathcal{E}
%\end{align*}


\begin{figure}[ht]
\centering
\begin{tikzpicture}[thick, color = black,
  %every node/.style={draw,circle},
  fsnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  ssnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  shorten >= 3pt,shorten <= 3pt
]

% the vertices of U

\begin{scope}[start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4}
  \node[fsnode,on chain] (r\i) [label=above left: {\small$\tau_\i$} ] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=3cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (t\i) [label=above right: {\small$\gamma_\i$}] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=6cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (tt\i) [label=above left: {\small$\overline\gamma_\i$}] {};
\end{scope}

\begin{scope}[xshift=9cm,yshift=0cm,start chain=going below,node distance=34.5mm]
\foreach \i in {1,2}
  \node[ssnode,on chain] (c\i) [label=above right: {\small$\omega_\i$}] {};
\end{scope}

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=left: $\xi$] at (-2, -1.5) (source) {};

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=right: $\overline\xi$ ] at (11, -1.8) (sink) {};

% the set U
%\node [blue,fit=(f1) (f5),label=above:$U$] {};
% the set V
%\node [green,fit=(s6) (s9),label=above:$V$] {};

% the edges

\foreach \i in {1,2,3,4} {
   \draw[color=gray] (source) -- (r\i);
   }

\foreach \i in {1,2,3,4} {
   \foreach \j in {1,2,3,4,5} {
   \draw[color=gray] (r\i) -- (t\j);
   }
 } 
 
\foreach \i in {1,2,3,4,5} {
   \draw[color=gray] (t\i) -- (tt\i);
}  
 
\foreach \i in {1,2,3,4,5} {
   \foreach \j in {1,2} {
   \draw[color=gray] (tt\i) -- (c\j);
   }
} 

\foreach \i in {1,2} {
   \draw[color=gray] (c\i) -- (sink);
}

% \node[text width=2cm, align = center] at (0,1.5) {\small\textsf{Black men patients}};
% \node[text width=2cm, align = center] at (3,1.5) {\small\textsf{White men patients}};
% \node[text width=2cm, align = center] at (6,1.5) {\small\textsf{Mirror White men patients}};
% \node[text width=2cm, align = center] at (9,1.5) {\small\textsf{Mirror Black men patients}};

\end{tikzpicture}
\caption{A basic illustrative plot of a generic tripartite network for matching with two criteria.
consisting of four units and five potential control units.}
\label{fig: tripartite network}
\end{figure}


\subsection{Connection to previous works}
\label{subsec: connection to previous works}
A tripartite network structure has been leveraged in the literature in two distinct contexts. \citet{zhang2021matching} proposed to use a tripartite network structure to construct matched pairs (or matched sets in general) from the set of treated units $\mathcal{T}$ and control units $\mathcal{C}$ that are (i) closely matched in key covariates; and (ii) balanced in high-dimensional covariates including the propensity score distributions. To achieve this using the network infrastructure described in Section \ref{subsec: tripartite structure}, simply let $\mathcal{A} = \mathcal{T}$ and $\mathcal{B} = \mathcal{T}$, so that vertices $\omega$ in Figure \ref{fig: tripartite network} become mirror copies of treated units and are now denoted as $\overline\tau$ instead. In other words, treated units appear twice in the network, in the far left and far right, and the control units are sandwiched between them. Figure \ref{fig: fine balance network} illustrates the network where the sample to be matched consists of $3$ treated units and $5$ control units. \citet{zhang2021matching} advocated equating $\delta(\tau_t, \gamma_c)$ to a measure of covariate similarity like the Mahalanobis distance or a robust version of it, and designing $\Delta(\tau_t, \gamma_c)$ in a way that minimizes the Earth Mover's distance between the estimated propensity score distributions of the treated group and the matched control group. We direct interested readers to Supplemental Material \textcolor{purple}{XX} for additional details. Under this framework, the final treated-to-control matched pairs can be obtained from flow $f$ as follows:
\begin{equation*}
    \mathcal{M}(f) = \left\{(\tau_t, \gamma_c), (\overline\gamma_c, \overline\tau_t)\in \mathcal{E}: f\{(\tau_t, \gamma_c)\} = f(\overline\gamma_c, \overline\tau_t)= 1\right\}.
\end{equation*}

\begin{figure}[ht]
\centering
\begin{tikzpicture}[thick, color = black,
  %every node/.style={draw,circle},
  fsnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  ssnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  shorten >= 3pt,shorten <= 3pt
]

% the vertices of U

\begin{scope}[start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[fsnode,on chain] (r\i) [label=above left: {\small$\tau_\i$} ] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=3cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (t\i) [label=above right: {\small$\gamma_\i$}] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=6cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (tt\i) [label=above left: {\small$\overline\gamma_\i$}] {};
\end{scope}

\begin{scope}[xshift=9cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[ssnode,on chain] (c\i) [label=above right: {\small$\overline\tau_\i$}] {};
\end{scope}

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=left: $\xi$] at (-2, -0.9) (source) {};

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=right: $\overline\xi$ ] at (11, -0.9) (sink) {};

% the set U
%\node [blue,fit=(f1) (f5),label=above:$U$] {};
% the set V
%\node [green,fit=(s6) (s9),label=above:$V$] {};

% the edges

\foreach \i in {1,2,3} {
   \draw[color=gray] (source) -- (r\i);
   }

\foreach \i in {1,2,3} {
   \foreach \j in {1,2,3,4,5} {
   \draw[color=gray] (r\i) -- (t\j);
   }
 } 
 
\foreach \i in {1,2,3,4,5} {
   \draw[color=gray] (t\i) -- (tt\i);
}  
 
\foreach \i in {1,2,3,4,5} {
   \foreach \j in {1,2,3} {
   \draw[color=gray] (tt\i) -- (c\j);
   }
} 

\foreach \i in {1,2,3} {
   \draw[color=gray] (c\i) -- (sink);
}

\end{tikzpicture}
\caption{A basic illustrative plot of a tripartite network consisting of three treated units and five potential control units.}
\label{fig: fine balance network}
\end{figure}

More recently, \citet{zhang2022towards} used a tripartite network to construct closely matched pairs from treated units $\mathcal{T}$ and control units $\mathcal{C}$ that further resemble a template $\mathcal{R}$ from a target population. To achieve this, let $\mathcal{A} = \mathcal{R}$, $\mathcal{C} = \mathcal{T}$ and $\mathcal{B} = \mathcal{C}$. See Figure \ref{fig: template matching network} for an example where there are $3$ treated units and $5$ control units, and researchers further have a template consisting of $2$ units. Under this framework, costs associated with edges $e(\kappa_r, \tau_t)$ facilitates selecting treated units resembling the template while costs associated with edges $e(\overline\tau_t, \gamma_c)$ facilitates the actual pair matching between treated and control units. \citet{zhang2022towards} advocated adding a large penalty to the right part of the network so that the internal validity of the matched sample is maximally maintained before pursuing its generalizability towards the target population. We refer interested readers to Supplemental Material \textcolor{purple}{XX} for additional details. In Figure \ref{fig: template matching network}, a pair-matched sample $\mathcal{M}(f)$ is defined as:
\begin{equation*}
    \mathcal{M}(f) = 
    \Big \{
    (\tau_t, \gamma_c) \in \mathcal{E}: f\{(\overline\tau_t, \gamma_c)\} = 1 \Big \}.
\end{equation*}

%Assume that each unit in the RCT, denoted by $\kappa_r$, is linked to a set of covariates represented by the vector $\widetilde{\boldsymbol{x}}$. Additionally, the original treated and control units are linked to a set of covariates that include both $\widetilde{\boldsymbol{x}}$ and another set of covariates denoted by $\boldsymbol{x}$, which are not available for the RCT units.


\begin{figure}[h]
\centering
\begin{tikzpicture}[thick, color = black,
  %every node/.style={draw,circle},
  fsnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  ssnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  shorten >= 3pt,shorten <= 3pt
]

% the vertices of U

\begin{scope}[start chain=going below,node distance=7mm]
\foreach \i in {1,2}
  \node[fsnode,on chain] (r\i) [label=above left: {\small$\kappa_\i$} ] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=3cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[ssnode,on chain] (t\i) [label=above right: {\small$\tau_\i$}] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=6cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[ssnode,on chain] (tt\i) [label=above left: {\small$\overline\tau_\i$}] {};
\end{scope}

\begin{scope}[xshift=9cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (c\i) [label=above right: {\small$\gamma_\i$}] {};
\end{scope}

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=left: $\xi$] at (-2, -0.5) (source) {};

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=right: $\overline\xi$ ] at (11, -1.9) (sink) {};

% the set U
%\node [blue,fit=(f1) (f5),label=above:$U$] {};
% the set V
%\node [green,fit=(s6) (s9),label=above:$V$] {};

% the edges

\foreach \i in {1,2} {
   \draw[color=black, line width = 0.5mm] (source) -- (r\i);
   }

\foreach \i in {1,2} {
   \foreach \j in {1,2,3} {
   \draw[color=gray] (r\i) -- (t\j);
   }
 } 

\draw[color = black, line width = 0.5mm] (r1) -- (t3);
\draw[color = black, line width = 0.5mm] (r2) -- (t1);

\foreach \i in {1,2,3} {
   \draw[color=gray] (t\i) -- (tt\i);
}

\draw[color = black, line width = 0.5mm] (t3) -- (tt3);
\draw[color = black, line width = 0.5mm] (t1) -- (tt1);
 
\foreach \i in {1,2,3} {
   \foreach \j in {1,2,3,4,5} {
   \draw[color=gray] (tt\i) -- (c\j);
   }
} 
\draw[color = black, line width = 0.5mm] (tt3) -- (c2);
\draw[color = black, line width = 0.5mm] (tt1) -- (c4);

\foreach \i in {1,2,3,4,5} {
   \draw[color=gray] (c\i) -- (sink);
}

\draw[color = black, line width = 0.5mm] (c2) -- (sink);
\draw[color = black, line width = 0.5mm] (c4) -- (sink);

\node[text width=2cm, align = center] at (0,1.5) {\small\textsf{Template}};
\node[text width=2cm, align = center] at (3,1.5) {\small\textsf{Treated}};
\node[text width=2cm, align = center] at (6,1.5) {\small\textsf{Treated}};
\node[text width=2cm, align = center] at (9,1.5) {\small\textsf{Control}};

\end{tikzpicture}
\caption{A basic illustrative network of a tripartite pair matching consisting of two template units, three treated units and five potential control units. The bold black lines correspond to two optimal matched pairs: ($\tau_1$, $\gamma_4$), ($\tau_3$, $\gamma_2$).}
\label{fig: template matching network}
\end{figure}



%Each treated unit is to be matched to $k$ control units among $C \geq T$ potential control available and each control appears at most once in matched comparisons. Fine balance or near-fine balance can be further achieved using the Earth Mover's distance \citep{levina2001earth}. The Earth Mover's distance measures the minimum amount of ``work" needed to transform one marginal distribution into the other, where ``work" is defined as the amount of probability mass (``earth") moved multiplied by the distance it is moved. While compared with related methods measuring the distance between nominal variables, such as Hamming distance, Earth Mover's distance achieves versatility by  not only measuring the distance between marginal distributions over categories but accepting any specified distance between categories.
%Suppose all the individuals $\tau_t \text{ and } \gamma_c \text{ for } ~t = 1, \dots, T,~c = 1, \dots, C$ are all allocated into $N$ mutually exclusive nominal categories defined by function $v: \mathcal{T} \cup \mathcal{C} \xrightarrow[]{} \{1, \dots, N\}$, that is, unit $\tau_t$ is in category $v(\tau_t)$. Define $p_i = k |\{\tau_t \in \mathcal{T}:v(\tau_t) = i\} |$, $k$ times number of treated units in the category $i$ and $q_i = |\{\gamma_c \in \mathcal{C}:v(\gamma_c) = i\} |$, number of control units in the category $i$ accordingly. The Earth Mover's distance is then defined as $(kT)^{-1}\min \Big\{ \sum_{i = 1}^N\sum_{j = 1}^N h_{i j}d_{i j} \Big\}$.
%The integer $h_{i j} \geq 0$ which depicts the number of matched controls belonging to category $j$ that have been considered to fulfill the demand for $p_i$ controls in category $i$. It subjects to the constrains: $\sum_{j = 1}^Nh_{i j} \leq p_i$ and $\sum_{i = 1}^Nh_{i j} \leq q_j$. While $d_{i j} \geq 0$ is a distance between category $i$ and category $j$ where $d_{i i} = 0$ and $d_{i j} > 0 ~\text{if } i \neq j$. Suppose using the Hamming distance to measure the distance between categories, then $d_{i j} = 1$ in this case.
%If the fine balance is possible, $h_{i j} = 0$ for $i \neq j$ and $h_{i i } = p_i$. Then the Earth Mover's distance is 0 since $d_{i i} = 0$. However, in practice, near-fine balance is often pursued to minimize the overall deviation from fine balance or total imbalance.
%Thus, it's natural to connect the cost expression on the right side of the network defined in Section \ref{sec: tripartite structure} in the form of computing the Earth Mover's distance. Let $\Delta_{\overline\tau_t, \overline\gamma_c} = d_{i j}$ if $\overline\tau_t$ falls in category $i$ and $\overline\gamma_c$ falls in category $j$, so $v(\overline\tau_t) = i \text{ and } v(\overline\gamma_c) = j$. Then for one feasible flow $f$, $\sum_{(\overline\tau_t, \overline\gamma_c) \in \mathcal{M}(f)}\Delta_{\overline\tau_t, \overline\gamma_c} = 
%\sum_{i = 1}^N\sum_{j = 1}^N h_{i j}d_{i j}$ 
%where $h_{i j} = |\{(\overline\tau_t, \overline\gamma_c) \in \mathcal{M}(f):v(\overline\tau_t) = i , v(\overline\gamma_c) = j\}|$. Therefore, minimizing the total cost on the right side of the network over all feasible flows is equivalent to minimize the total deviation from fine balance, in other words, minimize the Earth Mover's distance.
%To further ensure comparability between treated subjects and their matched comparisons, we can minimize the distance between their propensity score distributions. Propensity score is then viewed as a scalar covariate capturing imbalance in the observed covariates. Each subject's propensity score is treated as an unique category and then balance a $\{(k + 1)T\}$-category covariate between the treated and control groups. In this generalized case, integer $h_{i j}$ is either 1, representing matching $j^{th}$ control to $i^{th}$ treated subject, or 0, otherwise. And $d_{i j}$ is the absolute propensity score differences between the $j^{th}$ control to $i^{th}$ treated subject.






%treated units $\mathcal{T} = \{\tau_1, \dots, \tau_T\}$ are represented twice in the network, by nodes labeled $\tau_t$ and $\overline\tau_t$, $t = 1, \dots, T$, and control units $\mathcal{C} = \{\gamma_1, \dots, \gamma_C\}$ are represented by nodes labeled $\gamma_c$, $c = 1, \dots, C$ with $\mathcal{T} \cap \mathcal{C} = \varnothing$ (Figure \ref{fig: fine balance network}). Each treated unit is to be matched to $k$ control units among $C \geq T$ potential control available and each control appears at most once in matched comparisons. Fine balance or near-fine balance can be further achieved using the Earth Mover's distance \citep{levina2001earth}. 

%a minimum-cost network flow algorithm built upon a tripartite graph for multivariate matching. The treated units appear twice on either end with control units sandwiched in between. The algorithm balances high-dimensional covariates on the right side of the graph, while finding close matches is represented on the left side. By separating the two objectives of close pairing and covariate balancing, the algorithm effectively delivers homogeneous matched samples across important covariates while maintaining good balance across other covariates.


%\subsection{Application I: minimizing the earth mover's distance in the propensity score distribution}
%To achieve a $1\text{-to-}k$ match based on two criteria proposed by \citeauthor{zhang2021matching}, within the network infrastructure describe in Section \ref{sec: tripartite structure}, $T$ treated units $\mathcal{T} = \{\tau_1, \dots, \tau_T\}$ are represented twice in the network, by nodes labeled $\tau_t$ and $\overline\tau_t$, $t = 1, \dots, T$, and control units $\mathcal{C} = \{\gamma_1, \dots, \gamma_C\}$ are represented by nodes labeled $\gamma_c$, $c = 1, \dots, C$ with $\mathcal{T} \cap \mathcal{C} = \varnothing$ (Figure \ref{fig: fine balance network}). 

%\subsection{Application II: enhancing a matched comparison's generalizability}
% motivation
%In order to enable more accurate comparisons between effect estimates derived from observational studies and randomized controlled trials (RCTs), it is crucial to design an observational study that can produce treated and matched control groups that are comparable to the RCT population in terms of baseline covariates. After some modifications, the above-mentioned algorithm can construct matched groups that closely resemble a template, or a random sample from the target population, in key covariates.

%We provide a basic template matching example in Figure \ref{fig: template matching network}. Comparing to the original tripartite network structure in Figure \ref{fig: tripartite network}, we substitute the far left part vertex with $R$ template(RCT) units $\mathcal{K} = \{\kappa_1, .., \kappa_R\}$.
%The cost associated with edges $(\kappa_r, \tau_t)$ on the left network in Figure \ref{fig: template matching network} helps select treated units using RCT units as a template, while the right part of the network performs the actual statistical matching and returns a matched sample.
%A pair-matched sample $\mathcal{M}^\prime(f)$ is now defined as

%\begin{equation*}
%    \mathcal{M}^\prime(f) = 
%    \Big \{
%    (\tau_t, \gamma_c) \in \mathcal{E}: f\{(\tau_t, \gamma_c)\} = f\{(\overline\tau_t, \gamma_c)\} = 1 \mid f\{( \kappa_r, \tau_t )\} = 1
%    \Big \}
%\end{equation*}
%Assume that each unit in the RCT, denoted by $\kappa_r$, is linked to a set of covariates represented by the vector $\widetilde{\boldsymbol{x}}$. Additionally, the original treated and control units are linked to a set of covariates that include both $\widetilde{\boldsymbol{x}}$ and another set of covariates denoted by $\boldsymbol{x}$, which are not available for the RCT units.

%The cost of one feasible flow now can be written as:
%\begin{equation}\label{eq: template flow cost}
%    \text{cost}(f) = \sum_{\substack{(\kappa_r, \tau_t) \in \mathcal{E}: \\f\{(\kappa_r, \tau_t)\} = 1}} \delta_{\kappa_r, \tau_t} (\widetilde{\boldsymbol{x}}) ~+ \lambda \Big\{
%     \sum_{(\overline\tau_t, \gamma_c) \in \mathcal{M}^\prime(f)} \Delta_{\overline\tau_t, \gamma_c}\{(\widetilde{\boldsymbol{x}}, \boldsymbol{x})\} \Big\}
%\end{equation}
%Similar to equation \ref{eq: tripartite flow cost}, the total cost on the right side of expression \ref{eq: template flow cost} measures the degree of homogeneity between the treated and control groups that have been matched. However, in this case, the total cost on the left side of the network assesses how well the matched pairs represent the overall target population. A lower cost means that the matched cohort study can be generalized better to the target population.
%By further adjusting the value of $\lambda$ in this expression, we can focus either on the internal validity or the generalizability of the matched cohort study. In particular, a larger value of $\lambda$ will prioritize internal validity, whereas a smaller value emphasize on generalizability to the target RCT population. A properly chosen $\lambda$ value can help balance these two considerations.

%\textcolor{red}{illustrate with figure example }



\newpage

\section{A matched design for health disparities research}\label{sec: disparity_match_design}
\subsection{Adapting the tripartite network structure to constructing nested matched comparisons}
In the example about prostate cancer screening from Section \ref{sec: motivate example}, one could construct black and white patient groups that have similar distributions of all observed covariates with Application one. In empirical studies, researchers might also be interested in assessing the effects induced by one covariate subset, such as the covariates related to socioeconomic status in this case. It is straightforward to match only covariates except for socioeconomic status with Application One but this match can't ensure the accordance of socioeconomic status distribution between the match comparisons and unmatched white patients. 
Thus, we utilize this tripartite network structure to achieve two goals (i) to construct black-and-white patient pairs that are homogeneous in their biological covariates (Age, BMI, health status and smoking ) and (ii) the matched comparisons resemble the socioeconomic status covariates distributions of the unmatched white patient population.


\begin{figure}[ht]
\centering
\begin{tikzpicture}[thick, color = black,
  %every node/.style={draw,circle},
  fsnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  ssnode/.style={circle, fill=black, inner sep = 0pt, minimum size = 5pt},
  shorten >= 3pt,shorten <= 3pt
]

% the vertices of U

\begin{scope}[start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[fsnode,on chain] (r\i) [label=above left: {\small$\tau_\i$} ] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=3cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (t\i) [label=above right: {\small$\gamma_\i$}] {};
\end{scope}

% the vertices of V
\begin{scope}[xshift=6cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3,4,5}
  \node[ssnode,on chain] (tt\i) [label=above left: {\small$\overline\gamma_\i$}] {};
\end{scope}

\begin{scope}[xshift=9cm,yshift=0cm,start chain=going below,node distance=7mm]
\foreach \i in {1,2,3}
  \node[ssnode,on chain] (c\i) [label=above right: {\small$\gamma_\i^\prime$}] {};
\end{scope}

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=left: $\xi$] at (-2, -0.9) (source) {};

\node [circle, fill = black, inner sep = 0pt, minimum size = 5pt, label=right: $\overline\xi$ ] at (11, -0.9) (sink) {};

% the set U
%\node [blue,fit=(f1) (f5),label=above:$U$] {};
% the set V
%\node [green,fit=(s6) (s9),label=above:$V$] {};

% the edges

\foreach \i in {1,2,3} {
   \draw[color=black, line width = 0.5mm] (source) -- (r\i);
   }

\foreach \i in {1,2,3} {
   \foreach \j in {1,2,3,4,5} {
   \draw[color=gray] (r\i) -- (t\j);
   }
 }
 
\draw[color=black, line width = 0.5mm] (r1) -- (t3);
\draw[color=black, line width = 0.5mm] (r2) -- (t1);
\draw[color=black, line width = 0.5mm] (r3) -- (t5);
 
\foreach \i in {1,2,3,4,5} {
   \draw[color=gray] (t\i) -- (tt\i);
}

\draw[color=black, line width = 0.5mm] (t3) -- (tt3);
\draw[color=black, line width = 0.5mm] (t1) -- (tt1);
\draw[color=black, line width = 0.5mm] (t5) -- (tt5);

\foreach \i in {1,2,3,4,5} {
   \foreach \j in {1,2,3} {
   \draw[color=gray] (tt\i) -- (c\j);
   }
} 

\draw[color=black, line width = 0.5mm] (tt3) -- (c1);
\draw[color=black, line width = 0.5mm] (tt1) -- (c3);
\draw[color=black, line width = 0.5mm] (tt5) -- (c2);

\foreach \i in {1,2,3} {
   \draw[color=gray] (c\i) -- (sink);
}

\draw[color=black, line width = 0.5mm] (c1) -- (sink);
\draw[color=black, line width = 0.5mm] (c3) -- (sink);
\draw[color=black, line width = 0.5mm] (c2) -- (sink);

% \node[text width=2cm, align = center] at (0,1.5) {\small\textsf{Black men patients}};
% \node[text width=2cm, align = center] at (3,1.5) {\small\textsf{White men patients}};
% \node[text width=2cm, align = center] at (6,1.5) {\small\textsf{Mirror White men patients}};
% \node[text width=2cm, align = center] at (9,1.5) {\small\textsf{Mirror Black men patients}};

\end{tikzpicture}
\caption{The tripartite network structure for investigating specified effects. Three treated units and five potential control units. The bold black lines correspond to three optimal matched pairs: ($\tau_1$, $\gamma_3$), ($\tau_2$, $\gamma_1$), ($\tau_3$, $\gamma_5$)}.
\label{fig: sequential match}
\end{figure}

\subsection{Implementation using the \textsf{R} package \textsf{match2C}}
See the tutorial.


\textcolor{red}{One subsection could be on the adaptive caliper, i.e., a larger caliper size for ``edge cases" but a smaller caliper size for well-overlapped areas.}

\textcolor{red}{
TODO
\begin{itemize}
    \item diagnostic choice of randomization ahead of outcome analysis
    \item separate matched barplot, propen distribution and balance table
    \item if-else for customize lambda
    \item scale the cost (simple counter-example code)
\end{itemize}
}
